Learning from a Learning User for Optimal Recommendations

In real-world recommendation problems, especially those with a formidably large item space, users have to gradually learn to estimate the utility of any fresh recommendations from their experience about previously consumed items. This in turn affects their interaction dynamics with the system and can invalidate previous algorithms built on the omniscient user assumption. In this paper, we formalize a model to capture such "learning users" and design an efficient system-side learning solution, coined Noise-Robust Active Ellipsoid Search (RAES), to confront the challenges brought by the non-stationary feedback from such a learning user. Interestingly, we prove that the regret of RAES deteriorates gracefully as the convergence rate of user learning becomes worse, until reaching linear regret when the user's learning fails to converge. Experiments on synthetic datasets demonstrate the strength of RAES for such a contemporaneous system-user learning problem. Our study provides a novel perspective on modeling the feedback loop in recommendation problems.

==> algorithm.tex <==
\section{Learning from Explorative Users' Revealed Preferences}\label{sec:algo}

%First, we present the system's strategy from a high level. Since the system only observes binary decisions from the user, the only way to identify the best arm is to track the history of recommendations and rejections in order to eliminate suboptimal arms. 
With stochastic rewards, we know $\mathbb{P}[\mu_i \in CI_{i,t}]$ almost always increases as the number of acceptances $n(t)$ grows. Therefore, the system can confidently  rule out a sub-optimal arm once it has collected a reasonable number of acceptances. In light of this, we devise a two-phase explore-then-exploit strategy for system learning: the system first accumulates a sufficient number of acceptances and then examines through the arm set to eliminate sub-optimal ones with a high confidence. % Next, we present the algorithm for the two phases in detail.

\begin{algorithm}[t]
   \caption{Phase-1 Sweeping}
   \label{alg:phase1_alg}
%   \begin{multicols}{2}
\begin{algorithmic}
   \STATE {\bfseries Input:} $K>0$, $\delta\in (0,1) ,N_1(\delta)>0$. 
%   \REPEAT
\STATE {\bfseries Initialization:} $F=[K]$,$ N=0, n_i=0, i\in[K].$

\REPEAT
    \STATE Recommend each item in $F$ once, and remove the rejected ones from $F$.
\UNTIL{$F$ is empty or the time step exceeds $N_1(\delta)$.}

\REPEAT
\STATE If $F$ is empty, reset $F= \{1,\cdots, K\};$
    \FOR{$i \in F$} 
    \STATE Recommend $i$ until rejected, then remove it from $F$.
\ENDFOR
\UNTIL{The time step exceeds $N_1(\delta)$.}

   \STATE {\bfseries Output:} number of acceptances for each arm $\{n_i\}_{i=1}^K$. 
\end{algorithmic}
% \end{multicols}
\end{algorithm}



\begin{algorithm}[t]
   \caption{Phase-2 Elimination}
   \label{alg:phase2_alg}
%   \begin{multicols}{2}
\begin{algorithmic}
   \STATE {\bfseries Input:} $K>0$, $\{n_i\}_{i=1}^K$ from Phase-1.
   \STATE {\bfseries Initialization:} $F=[K] $.
   \
   
   \WHILE{$|F|>1$}
   \STATE Recommend $a_t=\arg\min_{i\in[K]} n_i$ and update $n_{a_t}$.
   \STATE Remove $a_t$ from $F$ if rejected.
   \ENDWHILE
 
   \STATE {\bfseries Output:} $F$.
\end{algorithmic}
% \end{multicols}
\end{algorithm}

% \end{multicols}


The Phase-1 design is presented in Algorithm \ref{alg:phase1_alg}. Like standard bandit algorithms,  
%the system recommends each arm once to the user. Given our user behavior model, the user always accepts the first $K$ recommendations. Then, 
the system will execute an initialization procedure by sweeping through the arm set $F=[K]$ and then recommend each arm repeatedly until it collects exactly one rejection on each arm there.  This initialization stage is similar to the round-robin style pulls in  standard bandit algorithms (e.g., UCB1, $\epsilon$-Greedy). But the key difference is that our algorithm will initialize by collecting one rejection on each arm whereas standard bandit algorithm will initialize by collecting one pull (i.e., acceptance) on each arm. This is because rejections in our setup are more informative than acceptances to the system. % as the system only starts to compare arms after they have been rejected: it can never hope to differentiate those arms which have always been accepted. If the number of acceptances exceeds $N_1$ during the warm-up stage, Algorithm \ref{alg:phase1_alg} terminates. Otherwise, 
After initialization, Algorithm \ref{alg:phase1_alg} enters the main loop and do the following: keeps recommending the same arm until it gets rejected and then moves to another arm in $F$. After each arm gets rejected once, the system starts a new round by resetting $F=[K]$. This procedure continues until the total number of acceptances exceeds $N_1(\delta)$. 
This sweeping strategy reflects the principle of Phase-1: the system aims to collect a reasonable number of acceptances while minimizing the number of rejections by not recommending any risky arm. 
For the ease of analysis, we divide Phase-1 into different \emph{rounds} (indexed by $r$) by the time steps when the system resets $F$.  We will prove later that there is a tailored choice of $N_1(\delta)$ such that when the system enters Phase-2 with $N_1(\delta)$ acceptance, it can identify the best arm with probability $1-\delta$.

One might notice that the Phase-1 algorithm \ref{alg:phase1_alg} needs to recommend each arm at least once and also needs to recommend each arm repeatedly in the candidate set to the user. Now a natural question to ask is, how this design could be practical given the immense size of item pool in a practical recommender system. However, we note that an arm in our model can be viewed as a type/category of items, rather than just literally an individual item. Therefore, Algorithm \ref{alg:phase1_alg} should not be interpreted as recommending the same item repeatedly to a user, but instead recommending items from the same category or type. This is also the typical interpretation of arms in stochastic bandit literature. Moreover, consuming repeatedly each item in the candidate set is a typical requirement in the stochastic bandit problems, due to the observation noise. More specifically, under a stochastic reward setting, the realized reward at each time step is randomly drawn from an underlying reward distribution, and repeated interactions are necessary to pin down the distribution. 

We now present the design for Phase-2, as shown in Algorithm \ref{alg:phase2_alg}, which follows Phase-1 Sweeping. Here, the system executes arm elimination: always recommend the arm with the minimum number of acceptances; and eliminate an arm when it is rejected by the user, until there is only one arm left. We prove that the stopping time of Algorithm \ref{alg:phase2_alg} is finite with probability 1, and it outputs the best arm with probability $1-\delta$ when it terminates. We name our proposed two-phase algorithm  \textbf{B}est \textbf{A}rm \textbf{I}dentification under \textbf{R}evealed preferences, or BAIR for short. 

Next, we analyze BAIR by upper bounding its stopping time given fixed confidence $\delta$. Our main result is formalized in the following theorem.

\begin{theorem}%[The Upper Bound for BAIR]
\label{thm:upperbound2}
When $\Gamma$ is defined as in Eq \eqref{eq:trust}, with probability at least $1-2\delta$, the system   makes at most $$  O\Big(K^{\frac{1}{\alpha}}\delta^{-\frac{1}{\alpha}}+K^{1+\frac{1}{2\alpha}}\delta^{-\frac{1}{2\alpha}}\sqrt{\log\frac{K}{\delta}}+\frac{\alpha K}{\Delta_1^2}\log\frac{ K}{\delta \Delta_1}\Big)$$ recommendations and successfully identifies the best arm by running Algorithm \ref{alg:phase1_alg} and \ref{alg:phase2_alg}. 
\end{theorem}
Note that the upper bound on the number of rounds above is deterministic while not in expectation. The proof of Theorem \ref{thm:upperbound2} requires separate analysis for Phase-1 and Phase-2, which we discuss in the following subsections. At a high level, the first two terms in the bound come from the number of acceptances and rejections in Phase-1, and the last term corresponds to the number of acceptances in Phase-2. We decompose the bound in Theorem \ref{thm:upperbound2} in Table \ref{tb:upperbounds}.
\begin{table}[ht]
\vspace{-1mm}
\centering
\caption{Upper bounds on \#recommendations in Phase 1,2}
\begin{tabular}{c|c|c|c}
 \hline
 Phase & \# Acceptance & \# Rejection &  Prob. \\  \hline
 1 & $O(K^{\frac{1}{\alpha}}\delta^{-\frac{1}{\alpha}})$ & $O(K^{\frac{1+2\alpha}{2\alpha}}\delta^{-\frac{1}{2\alpha}}\log^{\frac{1}{2}}\frac{K}{\delta})$ & $1-\delta$ \\  \hline
 2 & $O(\frac{\alpha K}{\Delta_1^2}\log\frac{K}{\delta \Delta_1})$ & $K$ & $1-\delta$ \\ \hline
\end{tabular}
\vspace{-2mm}
\label{tb:upperbounds}
\end{table}

Note that there is a clear \emph{tradeoff} between the upper bounds in Phase-1 and Phase-2 in terms of $\alpha$: a smaller $\alpha$ increases the upper bound in Phase-1 but requires less number of recommendations in Phase-2, while a larger $\alpha$ ensures a lighter Phase-1 but would result in a more cumbersome Phase-2. This is expected because, e.g., when facing a highly explorative user (large $\alpha$), the system can easily accumulate sufficient acceptances in Phase-1. However, it will need more comparisons in Phase-2 to identify the best arm for such a highly explorative user. Theoretically, there exists an optimal $\alpha$ which minimizes the total number of recommendations; however, this is not particularly interesting to investigate in this paper, as $\alpha$ is not under the system's control, but a characterization of the user.

%the system has to spend more time in Phase-1 to accumulate sufficient explorations when facing a conservative user; on the other hand, it needs more comparisons in Phase-2 to identify the best arm when the user is highly explorative. Theoretically, there exists an optimal $\alpha$ which minimizes the total number of recommendations; however, this is not particularly interesting to investigate in this paper, as $\alpha$ is not under the system's control, but a characterization of the user.

% In the following sections, we will analyze BAIR by upper bounding its stopping time given fixed confidence $\delta$ for Phase-1 and Phase-2 separately. 

